FLASH: Faint Lenses from Associated Selection with Herschel

We report the ALMA Band 7 observations of 86 Herschel sources that likely contain gravitationally-lensed galaxies. These sources are selected with relatively faint 500 $\mu$m flux densities between 15 to 85 mJy in an effort to characterize the effect of lensing across the entire million-source Herschel catalogue. These lensed candidates were identified by their close proximity to bright galaxies in the near-infrared VISTA Kilo-Degree Infrared Galaxy Survey (VIKING) survey. Our high-resolution observations (0.15 arcsec) confirm 47 per cent of the initial candidates as gravitational lenses, while lensing cannot be excluded across the remaining sample. We find average lensing masses (log M/M$_{\odot}$ = 12.9 $\pm$ 0.5) in line with previous experiments, although direct observations might struggle to identify the most massive foreground lenses across the remaining 53 per cent of the sample, particularly for lenses with larger Einstein radii. Our observations confirm previous indications that more lenses exist at low flux densities than expected from strong galaxy-galaxy lensing models alone, where the excess is likely due to additional contributions of cluster lenses and weak lensing. If we apply our method across the total 660 sqr. deg. H-ATLAS field, it would allow us to robustly identify 3000 gravitational lenses across the 660 square degree Herschel ATLAS fields.

==> images.tex <==
\begin{figure*}
    \centering
\includegraphics[width=\linewidth]{images/1.png}
\includegraphics[width=\linewidth]{images/2.png}
\includegraphics[width=\linewidth]{images/3.png}
\includegraphics[width=\linewidth]{images/4.png}
\includegraphics[width=\linewidth]{images/5.png}
    \caption{Caption}
    \label{fig:sources1}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/6.png}
\includegraphics[width=\linewidth]{images/7.png}
\includegraphics[width=\linewidth]{images/8.png}
\includegraphics[width=\linewidth]{images/9.png}
\includegraphics[width=\linewidth]{images/10.png}
    \caption{Caption}
    \label{fig:sources2}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/11.png}
\includegraphics[width=\linewidth]{images/12.png}
\includegraphics[width=\linewidth]{images/13.png}
\includegraphics[width=\linewidth]{images/14.png}
\includegraphics[width=\linewidth]{images/15.png}
    \caption{Caption}
    \label{fig:sources3}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/16.png}
\includegraphics[width=\linewidth]{images/17.png}
\includegraphics[width=\linewidth]{images/18.png}
\includegraphics[width=\linewidth]{images/19.png}
\includegraphics[width=\linewidth]{images/20.png}
    \caption{Caption}
    \label{fig:sources4}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/21.png}
\includegraphics[width=\linewidth]{images/22.png}
    \caption{Caption}
    \label{fig:sources5}
\end{figure*}

